On Optimizing Interventions in Shared Autonomy

Shared autonomy refers to approaches for enabling an autonomous agent to collaborate with a human with the aim of improving human performance. However, besides improving performance, it may often also be beneficial that the agent concurrently accounts for preserving the user's experience or satisfaction of collaboration. In order to address this additional goal, we examine approaches for improving the user experience by constraining the number of interventions by the autonomous agent. We propose two model-free reinforcement learning methods that can account for both hard and soft constraints on the number of interventions. We show that not only does our method outperform the existing baseline, but also eliminates the need to manually tune a black-box hyperparameter for controlling the level of assistance. We also provide an in-depth analysis of intervention scenarios in order to further illuminate system understanding.

==> sections/lunar_lander.tex <==
For Lunar Lander with discrete action space, we use four simulated agents as pilot, laggy pilot, noisy pilot, sensor pilot and noop pilot, which correspond to figure \ref{fig:lander laggy}, \ref{fig:lander noisy}, \ref{fig:lander sensor}, \ref{fig:lander noop}.

\subsection{Laggy Pilot}
\begin{figure*}[h!]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBaseline_laggy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBudget_laggy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_laggy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_Adapting_laggy.pdf}
         \end{subfigure}
     \end{subfigure}
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBaseline_laggy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBudget_laggy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_laggy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_Adapting_laggy.pdf}
         \end{subfigure}
     \end{subfigure}
     \caption{The return, intervention rate and success rate of the laggy pilot assisted by the copilot trained with different parameters for different methods on Lunar Lander with discrete action space.}
     \label{fig:lander laggy}
\end{figure*}

\newpage

\subsection{Noisy Pilot}
\begin{figure*}[h!]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBaseline_noisy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBudget_noisy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_noisy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_Adapting_noisy.pdf}
         \end{subfigure}
     \end{subfigure}
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBaseline_noisy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBudget_noisy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_noisy.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_Adapting_noisy.pdf}
         \end{subfigure}
     \end{subfigure}
     \caption{The return, intervention rate and success rate of the noisy pilot assisted by the copilot trained with different parameters for different methods on Lunar Lander with discrete action space.}
     \label{fig:lander noisy}
\end{figure*}





\subsection{Sensor Pilot}
\begin{figure*}[h!]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBaseline_sensor.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBudget_sensor.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_sensor.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_Adapting_sensor.pdf}
         \end{subfigure}
     \end{subfigure}
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBaseline_sensor.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBudget_sensor.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_sensor.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_Adapting_sensor.pdf}
         \end{subfigure}
     \end{subfigure}
     \caption{The return, intervention rate and success rate of the sensor pilot assisted by the copilot trained with different parameters for different methods on Lunar Lander with discrete action space.}
     \label{fig:lander sensor}
\end{figure*}

\newpage

\subsection{Noop Pilot}
\begin{figure*}[h!]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBaseline_noop.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsBudget_noop.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_noop.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_returnsPenalty_Adapting_noop.pdf}
         \end{subfigure}
     \end{subfigure}
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBaseline_noop.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherBudget_noop.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_noop.pdf}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.05in}
             \includegraphics[width=\textwidth]{figures/lander/lander_otherPenalty_Adapting_noop.pdf}
         \end{subfigure}
     \end{subfigure}
     \caption{The return, intervention rate and success rate of the noop pilot assisted by the copilot trained with different parameters for different methods on Lunar Lander with discrete action space.}
     \label{fig:lander noop}
\end{figure*}


==> sections/super_mario.tex <==
\subsubsection{Noisy Pilot}
For Super Mario, we use noisy pilot, which corresponds to figure \ref{fig:mario noisy}.

\begin{figure*}[h!]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_returns_Baseline.svg}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_returns_Budget.svg}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_returns_Penalty.svg}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_returns_Penalty_Adapting.svg}
         \end{subfigure}
     \end{subfigure}
     \begin{subfigure}[t]{\textwidth}
         \centering
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_other_Baseline.svg}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_other_Budget.svg}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_other_Penalty.svg}
         \end{subfigure}
         \begin{subfigure}[t]{0.24\textwidth}
             \centering
             \vspace{0.01in}
             \includesvg[width=\textwidth]{figures/mario/mario_other_Penalty_Adapting.svg}
         \end{subfigure}
     \end{subfigure}
     \caption{The return, intervention rate and success rate of the noisy pilot assisted by the copilot trained with different parameters for different methods on Super Mario.}
     \label{fig:mario noisy}
\end{figure*}
